TT-Rec: Tensor Train Compression for Deep Learning Recommendation Models

The memory capacity of embedding tables in deep learning recommendation models (DLRMs) is increasing dramatically from tens of GBs to TBs across the industry. Given the fast growth in DLRMs, novel solutions are urgently needed, in order to enable fast and efficient DLRM innovations. At the same time, this must be done without having to exponentially increase infrastructure capacity demands. In this paper, we demonstrate the promising potential of Tensor Train decomposition for DLRMs (TT-Rec), an important yet under-investigated context. We design and implement optimized kernels (TT-EmbeddingBag) to evaluate the proposed TT-Rec design. TT-EmbeddingBag is 3 times faster than the SOTA TT implementation. The performance of TT-Rec is further optimized with the batched matrix multiplication and caching strategies for embedding vector lookup operations. In addition, we present mathematically and empirically the effect of weight initialization distribution on DLRM accuracy and propose to initialize the tensor cores of TT-Rec following the sampled Gaussian distribution. We evaluate TT-Rec across three important design space dimensions -- memory capacity, accuracy, and timing performance -- by training MLPerf-DLRM with Criteo's Kaggle and Terabyte data sets. TT-Rec achieves 117 times and 112 times model size compression, for Kaggle and Terabyte, respectively. This impressive model size reduction can come with no accuracy nor training time overhead as compared to the uncompressed baseline.

==> production.tex <==
\textcolor{blue}{Given the space constraint, do we want to consider saving this section for the future?}

Application of TT-Rec to a production recommendation scenario requires
additional challenges in configuration selection for TT-Rec in order to find
the right balance of memory capacity reduction and execution time without
sacrificing from the strict model quality requirements of recommendation models.

In typical uses cases of recommendation models at scale, there are various different model configurations composed of variety of sizes including small and large tables.
Furthermore, the size of the table does not necessarily indicates its access frequency, i.e. there can be small tables can accessed frequently and large tables that are accessed less frequently.
Accuracy loss in the orders of $\sim$0.1\% may not be  tolerable  for  recommendation  models  to achieve a higher throughput. These make deciding which table to compress another important hyper parameter given strict model quality requirements of recommendation models.

%We apply TT-Rec to a commonly used model in production at an industry setting.
%Table~\ref{tab:prod_results} compares the baseline model and TT-Rec
%compressed version.
%\alert{TODO: explain the slowdown}

%\begin{table}
%\centering
%\tabcolsep=0.11cm
%\begin{tabular}{|l|c|c|c|} 
%\cline{1-4}
%                              & \textbf{Baseline} & \textbf{TT-Rec} & \textbf{TT-Rec/Baseline}\\ \cline{1-4}
%\textbf{Memory Capacity}      & 91.2 GB     &     42 GB &   0.46  \\ \cline{1-4}
%\textbf{Execution Time}       & 91 ms/it    &   738 ms/it &  8.11 \\ \cline{1-4}
%\textbf{Training Accuracy}    & 77.224 \%   &   77.267 \% &  1.00 \\ \cline{1-4}
%\textbf{Test Accuracy}        & 76.591 \%    &   77.090  \% & 1.01  \\ \cline{1-4}
%\end{tabular}
%\caption{Baseline vs TT-Rec for a production model.}
%\label{tab:prod_results}
%\end{table}

%\subsection{Compression Strategy}
%\label{sec:compression_strategy}
%Recommendation models commonly contain multiple embedding tables of different
%sizes and determining which tables to compress is an important design decision since it both impacts model compression ratio and model quality.
%Compressing more embedding tables can achieve significantly higher model compression %ratios, while the accuracy loss could increase as well.
%In practice, some embedding tables appear to be more important than the others, and are queried more frequently during training. The weight updates are more intensive on the frequently queried embedding tables. Thus, we want to minimize the approximation error on the popular embedding tables to reduce the impact on model accuracy. For the large but not frequently accessed embedding tables, we can adopt a more aggressive compression strategy to reduce the memory capacity while maintaining a decent model accuracy.



